A Survey of Distributed Consensus Protocols for Blockchain Networks

Since the inception of Bitcoin, cryptocurrencies and the underlying blockchain technology have attracted an increasing interest from both academia and industry. Among various core components, consensus protocol is the defining technology behind the security and performance of blockchain. From incremental modifications of Nakamoto consensus protocol to innovative alternative consensus mechanisms, many consensus protocols have been proposed to improve the performance of the blockchain network itself or to accommodate other specific application needs. In this survey, we present a comprehensive review and analysis on the state-of-the-art blockchain consensus protocols. To facilitate the discussion of our analysis, we first introduce the key definitions and relevant results in the classic theory of fault tolerance which help to lay the foundation for further discussion. We identify five core components of a blockchain consensus protocol, namely, block proposal, block validation, information propagation, block finalization, and incentive mechanism. A wide spectrum of blockchain consensus protocols are then carefully reviewed accompanied by algorithmic abstractions and vulnerability analyses. The surveyed consensus protocols are analyzed using the five-component framework and compared with respect to different performance metrics. These analyses and comparisons provide us new insights in the fundamental differences of various proposals in terms of their suitable application scenarios, key assumptions, expected fault tolerance, scalability, drawbacks and trade-offs. We believe this survey will provide blockchain developers and researchers a comprehensive view on the state-of-the-art consensus protocols and facilitate the process of designing future protocols.

==> bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio-YangXiao}}]{Yang Xiao}
(S'17) is currently pursuing the Ph.D. degree with the Bradley Department of Electrical and Computer Engineering at Virginia Tech, supervised by Prof. Wenjing Lou. He received his B.S. degree from the School of Electrical and Information Engineering at Shanghai Jiao Tong University and M.S. degree from the Electrical Engineering and Computer Science Department at University of Michigan, Ann Arbor. His research interests lie in network security, blockchain, and IoT security.
\end{IEEEbiography}
\vskip -1.5in
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio-NingZhang}}]{Ning Zhang}
(M'11) received the Ph.D. degree from Virginia Tech in 2016. He is currently an Assistant Professor with the Department of Computer Science and Engineering, Washington University in St. Louis. Before that, he was with an industry as a cyber engineer and a technical lead for over ten years. His research focus is system security, which lies at the intersection of security, embedded systems, and computer architecture and software.
\end{IEEEbiography}
\vskip -1.5in
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio-WenjingLou}}]{Wenjing Lou}
(F'15) received the Ph.D. degree in electrical and computer engineering from the University of Florida in 2003. From 2003 to 2011, she was a Faculty Member with the Worcester Polytechnic Institute. She has been a Professor with Virginia Tech since 2011. From 2014 to 2017, she was the Program Director of the U.S. National Science Foundation, where she was involved in the Networking Technology and Systems Program and the Secure and Trustworthy Cyberspace Program. Her current research interests focus on privacy protection techniques in networked information systems and cross-layer security enhancement in wireless networks by exploiting intrinsic wireless networking and communication properties.
\end{IEEEbiography}
\vskip -1.5in
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio-ThomasHou}}]{Y. Thomas Hou}
(F'14) received the Ph.D. degree from the NYU Tandon School of Engineering (formerly Polytechnic University) in 1998. He joined Virginia Tech, Blacksburg, VA, USA, in 2002, where he is currently a Bradley Distinguished Professor of Electrical and Computer Engineering. From 1997 to 2002, he was a Member of Research Staff with Fujitsu Laboratories of America, Sunnyvale, CA, USA. His current research focuses on developing innovative solutions to complex science and engineering problems arising from wireless and mobile networks. He is also interested in wireless security. He has over 250 papers published in the IEEE/ACM journals and conferences. His papers were recognized by five best paper awards from the IEEE and two paper awards from the ACM. He holds five U.S. patents. He has authored/co-authored two graduate textbooks: Applied Optimization Methods for Wireless Networks (Cambridge University Press, in 2014) and Cognitive Radio Communications and Networks: Principles and Practices (Academic Press/Elsevier, in 2009). He was named an IEEE Fellow for contributions to modeling and optimization of wireless networks. He was/is on the editorial boards of a number of IEEE and ACM transactions and journals. He is the Steering Committee Chair of the IEEE INFOCOM Conference and a member of the IEEE Communications Society Board of Governors. He is also a Distinguished Lecturer of the IEEE Communications Society.
\end{IEEEbiography}
